CODE: Contrasting Self-generated Description to Combat Hallucination in Large Multi-modal Models

Large Multi-modal Models (LMMs) have recently demonstrated remarkable abilities in visual context understanding and coherent response generation. However, alongside these advancements, the issue of hallucinations has emerged as a significant challenge, producing erroneous responses that are unrelated to the visual contents. In this paper, we introduce a novel contrastive-based decoding method, COuntering DEscription Contrastive Decoding (CODE), which leverages self-generated descriptions as contrasting references during the decoding phase of LMMs to address hallucination issues. CODE utilizes the comprehensive descriptions from model itself as visual counterpart to correct and improve response alignment with actual visual content. By dynamically adjusting the information flow and distribution of next-token predictions in the LMM's vocabulary, CODE enhances the coherence and informativeness of generated responses. Extensive experiments demonstrate that our method significantly reduces hallucinations and improves cross-modal consistency across various benchmarks and cutting-edge LMMs. Our method provides a simple yet effective decoding strategy that can be integrated to existing LMM frameworks without additional training.

==> table/table_ablation_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Ablation Studies.}
% \vspace{-1mm}
\label{table:quantitative-gpt-assisted}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ll|ccc|cccccccccccc}
 \Xhline{3\arrayrulewidth}\rule{0pt}{9pt}

 &  & \multicolumn{3}{c|}{MMVP} & \multicolumn{12}{c}{LLaVABench(In-the-Wild)} \\ \midrule
\multirow{2}{*}{kld_alpha} & \multirow{2}{*}{kl_d} & \multirow{2}{*}{LLaVA-1.5} & \multirow{2}{*}{LLaVA-Next} & \multirow{2}{*}{InternVL} & \multicolumn{4}{c}{LLaVA-1.5} & \multicolumn{4}{c}{LLaVA-Next} & \multicolumn{4}{c}{InternVL}

\\ 





 &  &  &  &  & Conv & Detail & Comp & Overall & Conv & Detail & Comp & Overall & Conv & Detail & Comp & Overall \\ \hline
- & - & 34 & 42.67 & 51.33 & 73.6 & 56 & 76.7 & 70.6 &  &  &  &  & 79.7 & 86.1 & 89.5 & 85.7 \\
\multicolumn{1}{r}{1} & - & 32 &  &  & 68.2 & 56.8 & 73.9 & 67.9 &  &  &  &  &  &  &  &  \\
- & \multicolumn{1}{r|}{0.1} & 28 & 33.33 &  & 62.7 & 55.4 & 75.1 & 66.5 & 72.3 & 77.1 & 85.6 & 79.7 &  &  &  &  \\
\multicolumn{1}{r}{1} & \multicolumn{1}{r|}{0.1} & 28.67 &  &  & 61.8 & 57.4 & 74.4 & 66.4 &  &  &  &  &  &  &  & 




\\\Xhline{3\arrayrulewidth}\rule{0pt}{9pt}
\end{tabular}
}
\end{table}
